Second-Order Bilevel Optimization with Accelerated Convergence Rates

This paper studies second-order methods for nonconvex-strongly-convex bilevel optimization. We propose a novel fully second-order bilevel approximation method (FSBA) that achieves an iteration complexity of $\tilde{\mathcal{O}}(\epsilon^{-1.5})$ for finding the $(\epsilon, \mathcal{O}(\sqrt{\epsilon}))$ second-order stationary point of the hyper-objective function. Our results demonstrate that second-order methods can achieve an accelerated convergence rate than first-order methods in bilevel optimization. To address the heavy computational cost associated with the second-order oracle, we introduce a lazy variant of FSBA, called LFSBA, which reuses second-order information across several iterations. We prove that LFSBA exhibits better computational complexity than FSBA by a factor of $\sqrt{d}$, where $d$ is the dimension of the problem. We also apply a similar idea to nonconvex strongly-concave minimax optimization and propose the lazy minimax cubic-regularized Newton (LMCN) method with better computational complexity compared to existing second-order methods.

==> inexact.tex <==










% \begin{lemma}[\cite{Luo22finding}, Theorem 3]
% \label{lem:IFSBA_convergence}
% Under Assumption~\ref{assum:basic}, if we
% run Algorithm~\ref{alg:IFSBA} with $C_\sigma = 1/4$, $\delta' = \delta / T$, 
% $T = \left\lceil626 \left(\fL_{\lambda}^*(\fx_0)-\min_{\fx}\fL_{\lambda}^*(\fx)\right)\sqrt{M} \, \epsilon^{-1.5} \right\rceil$,
% and suppose $K_t^1$, $K_t^2$, $K_1'$ and $K_2'$ are sufficiently large such that the following condition
% \begin{align}
% \label{eq:inexact-cubic-iteration-cheby}
% \begin{aligned}
% \left\|\nabla \mathcal{L}_\lambda^*\!\left(\boldsymbol{x}_t\right)
%       - \g(\fx_t;\fy_t,\fw_t)\right\|
% &\le C_g \epsilon, \\
% \left\|\nabla^2 \mathcal{L}_\lambda^*\!\left(\boldsymbol{x}_t\right)
%       - \C(\fx_t;\fy_t,\fw_t)\right\|
% &\le \min\!\left\{ C_H \sqrt{M\epsilon}, \epsilon_{\mathrm{H}} L \right\}.
% \end{aligned}
% \end{align}

% hold with $C_g = 1/240$ and $C_H = 1/200$.
% Then the condition $\Delta_t \geq -\frac{1}{128} \frac{\epsilon^3}{M}$ in line~8 must hold within no more than 
% $T = O\left( \kappa^{2.5} \sqrt{\bar{\ell} }\, \epsilon^{-1.5} \right)$ iterations; 
% and the output $\hat{\boldsymbol{x}}$ is an $(\epsilon, \OM(\kappa^{2.5} \sqrt{\bar{{\ell}}\epsilon} ))$-SOSP of $\fL^*_{\lambda}(\cdot)$
% with probability at least $1 - \delta$.
% \end{lemma}


We provide the following lemma to satisfy the condition~\eqref{eq:inexact-cubic-iteration-cheby}.

\begin{lemma}
\label{lem:IFSBA_inner_complexity}
Under Assumption~\ref{assum:basic}, let $\tilde{\epsilon} = \min\left\{ \frac{C_g \epsilon}{2\lambda\ell},\; \frac{\min\{ C_H \sqrt{M\epsilon} , \epsilon_{\mathrm{H}}L \}}{4 \textcolor{red}{C_2}} \right\}$, $R=\max(\left\|\fy^*\left(\boldsymbol{x}_0\right)\right\|, \left\|\fy_\lambda^*\left(\boldsymbol{x}_0\right)\right\|)$, and $\Delta=\varphi\left(\boldsymbol{x}_0\right) -\varphi^{*}$, 
if we run Algorithm~\ref{alg:IFSBA} with the same setting in Lemma~\ref{lem:IFSBA_convergence} and $\lambda = \max \left\{ \bar{\ell} \kappa^2 / \Delta, \bar{\ell}\kappa^3 / \epsilon, \bar{\ell}\kappa^5 / \sqrt{M\epsilon}\right\}$, $\kappa_1 = \kappa$, $\ell_1 = \ell$, $\kappa_2 = 3\kappa$, $\ell_2 = (1+\lambda)\ell$,
the order $K_1', K_2'$ of Chebyshev Polynomials in \eqref{eq:construct_cheby} as
\begin{equation*}
K_1'=K_2' = \frac{\sqrt{3\kappa} + 1}{2} \log\left( \frac{24(\lambda+1)\kappa \ell}{ \min\{ C_H \sqrt{M\epsilon} , \epsilon_{\mathrm{H}} L\}} \right)   
\end{equation*}
and the number of iterations of AGD subroutine as 
\begin{align*}
 K_t^1 = K_t^2 =\begin{cases}
    & \left\lceil 2 \sqrt{3\kappa} \log \left(\frac{\sqrt{3\kappa+1}}{\tilde{\epsilon}}R\right)\right\rceil~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~t=0 \\[0.3cm]
     & \left\lceil 2 \sqrt{3\kappa} \log \left(\frac{\sqrt{3\kappa+1}}{\tilde{\epsilon}}\left(\tilde{\epsilon}+4\kappa\left\|\boldsymbol{x}_t-\boldsymbol{x}_{t-1}\right\|\right)\right)\right\rceil~~~t\geq 1
 \end{cases},
\end{align*}
then the condition \eqref{eq:inexact-cubic-iteration-cheby} in Lemma~\ref{lem:IFSBA_convergence} is satisfied. 

Note that the value of $K' = O(\sqrt{\kappa})$ corresponds to the number of Hessian-vector product calls per iteration of the cubic subproblem solver (Algorithms~\ref{alg:cubic_sub} and~\ref{alg:final_cubic}). Combining Lemma~\ref{lem:IFSBA_convergence}, Lemma~\ref{lem:IFSBA_inner_complexity}, and the value of $\mathcal{K}(\epsilon, \delta')$, we obtain the main result for Algorithm~\ref{alg:IFSBA} as follows.
\end{lemma}






\begin{theorem}
\label{thm:imcn_main_complexity}
Under Assumption~\ref{assum:basic}, run Algorithm~\ref{alg:IFSBA} under the same setting as in Lemma~\ref{lem:IFSBA_convergence} and \ref{lem:IFSBA_inner_complexity}, let $M=\Omega( \bar{\rho})$, 
$T = \Theta((\varphi(\fx_0)-\varphi^*)\sqrt{M}\epsilon^{-3/2})$, then
$\hat{\fx}$ is an $((\OM(\epsilon),\OM(\kappa^{2.5}\bar{\ell}^{0.5}\epsilon^{0.5}))$-SOSP of $\varphi(\cdot)$ with probability at least $1 - \delta$. In addition, the total number of $K^1_t$, $K^2_t$ can be bounded by
$  \sum_{t=0}^{T-1}(K^1_t+K^2_t) \leq \tilde{\OM}(\kappa^3\bar{\ell}^{0.5}\epsilon^{-1.5}).$
The complexities of the gradient calls and Hessian-vector product calls can be bounded by $\tilde{\OM}(\kappa^3\bar{\ell}^{0.5}\epsilon^{-1.5})$ and ${\OM}(\kappa^{3.5}\bar{\ell}\epsilon^{-2})$, respectively.
\end{theorem}

\begin{algorithm}
\caption{Final-Cubic-Solver}
\label{alg:final_cubic}
\begin{algorithmic}[1]
\STATE \textbf{Input:} $\g, \H, \epsilon$
\vskip 0.2cm
\STATE $\boldsymbol{s}_0 = \mathbf{0},\ \g_0 = \g,\ \eta = 1/(20L)$
\FOR{$t = 0, 1, \cdots$}
    \IF{$\|\g_t\| \leq \epsilon / 2$}
        \STATE \textbf{break}
    \ENDIF
    \STATE $\boldsymbol{s}_{t+1} = \boldsymbol{s}_t - \eta \g_t$
    \STATE $\g_{t+1} = \g + \H \boldsymbol{s}_{t+1} + \dfrac{M}{2} \|\boldsymbol{s}_{t+1}\|\boldsymbol{s}_{t+1}$
\ENDFOR
\vskip 0.2cm
\STATE \textbf{Output:} $\hat{\boldsymbol{s}} = \boldsymbol{s}_t$
\end{algorithmic}
\end{algorithm}

% \section{Numerical Experiments}
% \label{sec:exp}

% \subsection{Data Hypercleaning}
% \begin{figure*}[t] % 必须是 figure* 以跨双栏
%     \centering
%     % 收紧列间距，把空间留给图片
%     \setlength{\tabcolsep}{1pt} 
    
%     \begin{tabular}{cccc} % 改为四列 cccc
%         % 第一行：四张图片
%         \includegraphics[width=0.24\linewidth]{figures/breast-25.png} &
%         \includegraphics[width=0.24\linewidth]{figures/breast-50.png} &
%         \includegraphics[width=0.24\linewidth]{figures/australian-25.png} &
%         \includegraphics[width=0.24\linewidth]{figures/australian-50.png} \\
        
%         % 第二行：四个小标题 (使用 \scriptsize 防止文字换行)
%         \scriptsize Breast $p=0.25$ & 
%         \scriptsize Breast $p=0.5$ &
%         \scriptsize Australian $p=0.25$ & 
%         \scriptsize Australian $p=0.5$
%     \end{tabular}
    
%     \vspace{-0.5em} % 稍微减少一点图片和主标题之间的空白
%     \caption{Comparison of various bilevel algorithms with different noise rate $p$ on ``breast-cancer'' and ``australian'' datasets.}
%     \label{fig:data hyper}
% \end{figure*}

% We conduct experiments to validate the efficiency of the proposed methods on the \textit{data hyper-cleaning} task~\cite{franceschi2018bilevel,shaban2019truncated,zhou2022model}, which can be formulated as a bilevel optimization problem~\eqref{eq:bilevel} with  the following 
% upper and lower-level objectives:
% {\small
% \begin{equation}
% \begin{split}
%     f(\fx, \fy) &:= \frac{1}{|\mathcal{D}^{\mathrm{val}}|} \sum_{(\va_i, b_i) \in \mathcal{D}^{\mathrm{val}}} \ell(\langle \va_i, \fy\rangle, b_i), \\
%     g(\fx, \fy) &:= \frac{1}{|\mathcal{D}^{\mathrm{tr}}|} \sum_{(\va_i, b_i) \in \mathcal{D}^{\mathrm{tr}}} \sigma(x_i) \ell(\langle \va_i, \fy\rangle, b_i) + c\|\fy\|^2.
% \end{split}
% \end{equation}
% }
% In the above, $\mathcal{D}^{\operatorname{tr}}$ denotes the noisy training set and $\mathcal{D}^{\mathrm{val}}$ denotes the validation set. $\left(\va_i, b_i\right)$ denotes the $i$-th sample in the dataset, where $\va_i$ represents the feature and $b_i$ represents its corresponding label. 
% We denote $\sigma(\cdot)$ as a clipping function that maps a scalar to the interval $[0,1]$ and $\ell(\cdot, \cdot)$ is the loss of cross entropy.
% We set $c=10^{-3}$.

% For low-dimensional cases, we compare the LSFBA method (Algorithm~\ref{alg:LFSBA}) with baseline methods, including ITD~\cite{ji2021bilevel}, AID with conjugate gradient~\cite{maclaurin2015gradient}, and F$^2$BA~\cite{Chen23Nearoptimal} on "breast-cancer" and "australian" datasets~\cite{chang2011libsvm}.
% We report the results on $\fD_{tr}$ with different noise rates $p  = 25\%$ and $p = 50\%$ (the ratio of training samples with disrupted labels) in Figure~\ref{fig:data hyper}. We tune the learning rate for AID, ITD, F$^2$BA, and the AGD steps in LFSBA by selecting from the set $\left\{10^3, 10^2, 10^1, 10^0, 10^{-1}, 10^{-2}, 10^{-3}\right\}$. 
% For F$^2$BA and LFSBA, we additionally tune the multiplier $\lambda$ in $\left\{10^1, 10^2, 10^3\right\}$. 
% For LFSBA, we tune $M$ from $\left\{10^1, 10^2, 10^3\right\}$ and $m$ from $\{1,5,10,100\}$. 

% For high-dimensional cases, we compare IFSBA method (Algorithm~\ref{alg:IFSBA}) with baseline methods, including ITD, AID with conjugate gradient, and F$^2$BA on "MNIST" datasets~\cite{lecun2002gradient}. We report the results on $\fD_{tr}$ with different noise rates $p  = 25\%$ and $p = 50\%$ in Figure~\ref{fig:MNIST}. For hyperparameter selection, the settings follow the low-dimensional cases, except that IFSBA requires additional tuning of the Cubic-Solver iterations and Matrix Chebyshev Polynomials chosen from $\{1, 5, 10, 100\}$.


